GULP: a prediction-based metric between representations

Comparing the representations learned by different neural networks has recently emerged as a key tool to understand various architectures and ultimately optimize them. In this work, we introduce GULP, a family of distance measures between representations that is explicitly motivated by downstream predictive tasks. By construction, GULP provides uniform control over the difference in prediction performance between two representations, with respect to regularized linear prediction tasks. Moreover, it satisfies several desirable structural properties, such as the triangle inequality and invariance under orthogonal transformations, and thus lends itself to data embedding and visualization. We extensively evaluate GULP relative to other methods, and demonstrate that it correctly differentiates between architecture families, converges over the course of training, and captures generalization performance on downstream linear tasks.

==> Geometric Toolkit_arXiv/importsanddeclares.tex <==
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{color}
\usepackage{mathtools}
\usepackage{makecell}
\usepackage{bm}
\usepackage{todonotes}
\usepackage{diagbox}
\usepackage{tablefootnote}
\usepackage[colorlinks=true,linkcolor=blue]{hyperref}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{layouts}
\usepackage{algorithmic}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{color}
\usepackage{mathtools}
\usepackage{makecell}
\usepackage{bm}
\usepackage{todonotes}
\usepackage{diagbox}
\usepackage{tablefootnote}
\usepackage{fancybox}
\usepackage[bottom]{footmisc}
\usepackage{appendix}

\DeclarePairedDelimiter{\round}{\lceil}{\rfloor}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\DeclareMathOperator{\pa}{pa}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\LCA}{LCA}
\DeclareMathOperator{\coeff}{coeff}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\comp}{comp}
\DeclareMathOperator{\wt}{wt}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\SDP}{SDP}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Det}{det}
\DeclareMathOperator{\Perm}{perm}
\DeclareMathOperator{\Ima}{im}
\DeclareMathOperator{\Char}{char}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\Ber}{Ber}
\DeclareMathOperator{\Bern}{Bern}
\DeclareMathOperator{\Rad}{Rad}
\DeclareMathOperator{\Bin}{Bin}
\DeclareMathOperator{\Pois}{Pois}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\ReLU}{ReLU}
\DeclareMathOperator\tr{tr}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}


\let\vaccent=\v %
\renewcommand{\v}[1]{\ensuremath{\mathbf{#1}}} %
\newcommand{\gv}[1]{\ensuremath{\mbox{\boldmath$ #1 $}}} 
\newcommand{\uv}[1]{\ensuremath{\mathbf{\hat{#1}}}} %
\newcommand{\abs}[1]{\left| #1 \right|} %
\newcommand{\avg}[1]{\left< #1 \right>} %
\let\underdot=\d %
\renewcommand{\d}[2]{\frac{d #1}{d #2}} %
\newcommand{\dd}[2]{\frac{d^2 #1}{d #2^2}} %
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} 
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}} 
\newcommand{\pdc}[3]{\left( \frac{\partial #1}{\partial #2}
 \right)_{#3}} %
\newcommand{\ket}[1]{\left| #1 \right>} %
\newcommand{\bra}[1]{\left< #1 \right|} %
\newcommand{\braket}[2]{\left< #1 \vphantom{#2} \right|
 \left. #2 \vphantom{#1} \right>} %
\newcommand{\matrixel}[3]{\left< #1 \vphantom{#2#3} \right|
 #2 \left| #3 \vphantom{#1#2} \right>} %
\newcommand{\grad}[1]{\gv{\nabla} #1} %
\let\divsymb=\div %
\renewcommand{\div}[1]{\gv{\nabla} \cdot \v{#1}} %
\newcommand{\curl}[1]{\gv{\nabla} \times \v{#1}} %
\let\baraccent=\= %
\renewcommand{\=}[1]{\stackrel{#1}{=}} %
\providecommand{\wave}[1]{\v{\tilde{#1}}}
\providecommand{\fr}{\frac}
\providecommand{\tbf}{\textbf}
\providecommand{\tsc}{\textsc}
\providecommand{\RR}{\mathbb{R}}
\providecommand{\R}{\mathbb{R}}
\providecommand{\NN}{\mathbb{N}}
\providecommand{\CC}{\mathbb{C}}
\providecommand{\FF}{\mathbb{F}}
\providecommand{\LL}{\mathbb{L}}
\providecommand{\ZZ}{\mathbb{Z}}
\providecommand{\QQ}{\mathbb{Q}}
\providecommand{\cA}{\mathcal{A}}
\providecommand{\cB}{\mathcal{B}}
\providecommand{\cC}{\mathcal{C}}
\providecommand{\cD}{\mathcal{D}}
\providecommand{\cE}{\mathcal{E}}
\providecommand{\cF}{\mathcal{F}}
\providecommand{\cG}{\mathcal{G}}
\providecommand{\cL}{\mathcal{L}}
\providecommand{\cM}{\mathcal{M}}
\providecommand{\cN}{\mathcal{N}}
\providecommand{\cP}{\mathcal{P}}
\providecommand{\cR}{\mathcal{R}}
\providecommand{\cS}{\mathcal{S}}
\providecommand{\cV}{\mathcal{V}}
\providecommand{\cX}{\mathcal{X}}
\providecommand{\cY}{\mathcal{Y}}
\providecommand{\sH}{\mathsf{H}}
\providecommand{\sT}{\mathsf{T}}
\providecommand{\sT}{\mathsf{T}}
\providecommand{\PP}{\mathbb{P}}
\providecommand{\EE}{\mathbb{E}}
\providecommand{\fM}{\mathfrak{M}}
\providecommand{\seq}{\subseteq}
\providecommand{\e}{\epsilon}
\providecommand{\eps}{\epsilon}
\providecommand{\de}{\delta}
\providecommand{\La}{\Lambda}
\providecommand{\N}{\mathbb{N}}
\providecommand{\la}{\lambda}
\providecommand{\al}{\alpha}
\providecommand{\Al}{\Alpha}
\providecommand{\vareps}{\varepsilon}
\providecommand{\NTIME}{\mathsf{NTIME}}
\providecommand{\DTIME}{\mathsf{DTIME}}
\providecommand{\SigmaTIME}[1]{\mathsf{\Sigma_{#1}}\mathsf{TIME}}
\providecommand{\PiTIME}[1]{\mathsf{\Pi_{#1}}\mathsf{TIME}}
\providecommand{\PH}{\mathsf{PH}}
\renewcommand{\P}{\mathsf{P}}
\providecommand{\NP}{\mathsf{NP}}
\providecommand{\NSUBEXP}{\mathsf{NSUBEXP}}
\providecommand{\NEXP}{\mathsf{NEXP}}
\providecommand{\coNP}{\mathsf{coNP}}
\providecommand{\PSPACE}{\mathsf{PSPACE}}
\providecommand{\BPP}{\mathsf{BPP}}
\providecommand{\BPNP}{\mathsf{BP}\bm{\cdot}\mathsf{NP}}
\providecommand{\DP}{\mathsf{DP}}
\providecommand{\AM}{\mathsf{AM}}
\providecommand{\VP}{\mathsf{VP}}
\providecommand{\VQP}{\mathsf{VQP}}
\providecommand{\VNP}{\mathsf{VNP}}
\providecommand{\sharpP}{\mathsf{\#P}}
\providecommand{\Ppoly}{\mathsf{P/poly}}
\providecommand{\NPpoly}{\mathsf{NP/poly}}
\providecommand{\SIZE}{\mathsf{SIZE}}
\providecommand{\ASIZE}{\mathsf{ASIZE}}
\providecommand{\PERM}{\textsc{Perm}}
\providecommand{\PIT}{\textsc{PIT}}
\providecommand{\RP}{\mathsf{RP}}
\mathchardef\mhyphen="2D %
\providecommand{\complete}{\mathsf{\mhyphen complete}}
\providecommand{\hard}{\mathsf{\mhyphen hard}}
\providecommand{\co}{\mathsf{co}}
\newcommand{\Pcc}{\mathsf{P^{cc}}}
\newcommand{\Pdt}{\mathsf{P^{dt}}}
\newcommand{\NPdt}{\mathsf{NP^{dt}}}
\newcommand{\NPcc}{\mathsf{NP^{cc}}}
\newcommand{\UPcc}{\mathsf{UP^{cc}}}
\newcommand{\UPdt}{\mathsf{UP^{dt}}}


\newcommand{\BSC}{\mathsf{BSC}}
\newcommand{\AWGN}{\mathsf{AWGN}}
\newcommand{\iid}{\stackrel{\mathrm{IID}}{\sim}}

\providecommand{\ba}{\bm{a}}
\providecommand{\bb}{\bm{b}}
\providecommand{\bc}{\bm{c}}
\providecommand{\bd}{\bm{d}}
\providecommand{\be}{\bm{e}}
\providecommand{\br}{\bm{r}}
\providecommand{\bt}{\bm{t}}
\providecommand{\bw}{\bm{w}}
\providecommand{\bx}{\bm{x}}
\providecommand{\by}{\bm{y}}
\providecommand{\bG}{\bm{G}}
\providecommand{\bQ}{\bm{Q}}

\newcommand{\dec}{{\sf Dec}}
\newcommand{\gen}{{\sf Gen}}
\newcommand{\sign}{{\sf Sign}}
\newcommand{\ver}{{\sf Ver}}
\newcommand{\pk}{{\sf pk}}


\providecommand{\sm}{\setminus}
\providecommand{\parmu}{\partial_{\mu}}
\providecommand{\parnu}{\partial_{\nu}}
\providecommand{\is}[1]{\indices{#1}}
\providecommand{\cH}{\mathcal{H}}
\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
\newcommand\chr[3]{\Gamma^{#1}_{#2 #3}}
\newcommand{\Mod}[1]{\ (\text{mod}\ #1)}
\providecommand{\del}{\nabla}
\providecommand{\gen}[1]{\langle #1 \rangle}
\newcommand{\fl}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ce}[1]{\left\lceil #1 \right\rceil}
\providecommand{\lar}{\leftarrow}
\providecommand{\rar}{\rightarrow}
\providecommand{\lrar}{\leftrightarrow}
\newcommand{\interior}[1]{%
  {\kern0pt#1}^{\mathrm{o}}%
}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\providecommand{\indy}{\independent}




\usepackage[capitalise]{cleveref}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}



\providecommand{\cl}{\mathrm{cl}}





\providecommand{\editdist}{\mathrm{ed}}

\newcommand{\loctv}{\mathsf{locTV}}
\newcommand{\loctvk}[1]{\mathsf{locTV}^{(#1)}}
\newcommand{\muh}{{\hat \mu}}

\newcommand{\TCL}{\sT^{\mathsf{CL}}} %
\newcommand{\thetaCL}{\theta^{\mathsf{CL}}}
\providecommand{\dsT}{\dot{\sT}}
\providecommand{\tsT}{\tilde{\sT}}
\providecommand{\tsH}{\tilde{\sH}}
\providecommand{\dsH}{\dot{\sH}}
\providecommand{\hmu}{\hat{\mu}}
\providecommand{\tmu}{\tilde{\mu}}
\providecommand{\Thetah}{\hat{\Theta}}


\newcommand{\ReduceToFerromagnetic}{\texttt{LearnModel}}
\newcommand{\ReduceToLowerBounded}{\texttt{Reduce-To-Lower-Bounded}}
\newcommand{\FerromagneticSubroutine}{\texttt{LearnFerromagneticModel}}
\newcommand{\LowerboundedSubroutine}{\texttt{LowerboundedSubroutine}}
\newcommand{\ChowLiuPreprocessing}{\texttt{ChowLiuPartitioning}}
\newcommand{\LearnFerromagneticModel}{\texttt{LearnFerromagneticModel}}
\newcommand{\LearnLowerboundedModel}{\texttt{LearnLowerboundedModel}}
\newcommand{\GlobalReconstruction}{\texttt{LearnLowerboundedModel}}
\newcommand{\Desteinerize}{\texttt{Desteinerize}}

\renewcommand{\Im}{\mathrm{Im}}
\renewcommand{\Re}{\mathrm{Re}}

\newcommand{\vectorize}{\mathrm{vec}}
\newcommand{\fjunk}{f_{\mathrm{junk}}}
\newcommand{\Djunk}{\cD_{\mathrm{junk}}}
\newcommand{\elljunk}{\ell_{\Djunk}}

\newcommand{\tTheta}{\tilde{\Theta}}
\newcommand{\tilTh}{\tilde{\Theta}}
\newcommand{\tilW}{\tilde{W}}
\newcommand{\tilV}{\tilde{V}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\KL}{\mathrm{KL}}

\def\bA{{\boldsymbol A}}
\def\bB{{\boldsymbol B}}
\def\bC{{\boldsymbol C}}
\def\bD{{\boldsymbol D}}
\def\bE{{\boldsymbol E}}
\def\bF{{\boldsymbol F}}
\def\bG{{\boldsymbol G}}

\def\bH{{\boldsymbol H}}
\def\bI{{\boldsymbol I}}
\def\bJ{{\boldsymbol J}}
\def\bK{{\boldsymbol K}}
\def\bL{{\boldsymbol L}}
\def\bM{{\boldsymbol M}}
\def\bN{{\boldsymbol N}}
\def\bO{{\boldsymbol O}}
\def\bP{{\boldsymbol P}}
\def\bQ{{\boldsymbol Q}}
\def\bR{{\boldsymbol R}}
\def\bS{{\boldsymbol S}}
\def\bT{{\boldsymbol T}}
\def\bU{{\boldsymbol U}}
\def\bV{{\boldsymbol V}}
\def\bW{{\boldsymbol W}}
\def\bX{{\boldsymbol X}}
\def\bY{{\boldsymbol Y}}
\def\bZ{{\boldsymbol Z}}

\def\ba{{\boldsymbol a}}
\def\bb{{\boldsymbol b}}
\def\be{{\boldsymbol e}}
\def\boldf{{\boldsymbol f}}
\def\bg{{\boldsymbol g}}
\def\bh{{\boldsymbol h}}
\def\bi{{\boldsymbol i}}
\def\bj{{\boldsymbol j}}
\def\bk{{\boldsymbol k}}
\def\bq{{\boldsymbol q}}
\let\bsold\bs
\def\bs{{\boldsymbol s}}
\def\bt{{\boldsymbol t}}
\def\bu{{\boldsymbol u}}
\def\bv{{\boldsymbol v}}
\def\bw{{\boldsymbol w}}
\def\bx{{\boldsymbol x}}
\def\by{{\boldsymbol y}}
\def\bz{{\boldsymbol z}}

\def\bbeta{{\boldsymbol \beta}}
\def\balpha{{\boldsymbol \alpha}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol \eps}}
\def\blambda{{\boldsymbol \lambda}}
\def\bpsi{{\boldsymbol \psi}}
\def\bphi{{\boldsymbol \phi}}
\def\btheta{{\boldsymbol \theta}}
\def\tbtheta{\tilde{\btheta}}
\def\bvphi{{\boldsymbol \vphi}}
\def\bxi{{\boldsymbol \xi}}

\def\bDelta{{\boldsymbol \Delta}}
\def\bLambda{{\boldsymbol \Lambda}}
\def\bPsi{{\boldsymbol \Psi}}
\def\bPhi{{\boldsymbol \Phi}}
\def\bSigma{{\boldsymbol \Sigma}}
\def\bTheta{{\boldsymbol \Theta}}
\def\bzeta{{\boldsymbol \zeta}}

\def\bzero{{\boldsymbol 0}}
\def\bfzero{{\boldsymbol 0}}
\def\bfone{{\boldsymbol 1}}
\def\bone{{\boldsymbol 1}}


\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}

\newcommand{\fNN}{f_{\mathsf{NN}}}
\newcommand{\tfNN}{\tilde{f}_{\mathsf{NN}}}
\newcommand{\gNN}{g_{\mathsf{NN}}}

\newcommand{\barcF}{\bar{\cF}}

\newcommand{\fparity}{f_{\mathrm{parity}}}
\newcommand{\fmodeight}{f_{\mathrm{mod8}}}
\newcommand{\cDmodeight}{\cD_{\mathrm{mod8}}}

\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}

\newenvironment{algbox}[0]{
\noindent 
\begin{fminipage}{4.7in}
}{
\end{fminipage}
}


\newcommand{\ud}{\mathrm{d}}
\newcommand{\sig}{\sigma}

==> importsanddeclares.tex <==
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{color}
\usepackage{mathtools}
\usepackage{makecell}
\usepackage{bm}
\usepackage{todonotes}
\usepackage{diagbox}
\usepackage{tablefootnote}
\usepackage[colorlinks=true,linkcolor=blue]{hyperref}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{layouts}
\usepackage{algorithmic}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{color}
\usepackage{mathtools}
\usepackage{makecell}
\usepackage{bm}
\usepackage{todonotes}
\usepackage{diagbox}
\usepackage{tablefootnote}
\usepackage{fancybox}
\usepackage[bottom]{footmisc}
\usepackage{appendix}

\DeclarePairedDelimiter{\round}{\lceil}{\rfloor}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\DeclareMathOperator{\pa}{pa}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\LCA}{LCA}
\DeclareMathOperator{\coeff}{coeff}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\length}{length}
\DeclareMathOperator{\comp}{comp}
\DeclareMathOperator{\wt}{wt}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\SDP}{SDP}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Det}{det}
\DeclareMathOperator{\Perm}{perm}
\DeclareMathOperator{\Ima}{im}
\DeclareMathOperator{\Char}{char}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\Ber}{Ber}
\DeclareMathOperator{\Bern}{Bern}
\DeclareMathOperator{\Rad}{Rad}
\DeclareMathOperator{\Bin}{Bin}
\DeclareMathOperator{\Pois}{Pois}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator{\ReLU}{ReLU}
\DeclareMathOperator\tr{tr}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}


\let\vaccent=\v %
\renewcommand{\v}[1]{\ensuremath{\mathbf{#1}}} %
\newcommand{\gv}[1]{\ensuremath{\mbox{\boldmath$ #1 $}}} 
\newcommand{\uv}[1]{\ensuremath{\mathbf{\hat{#1}}}} %
\newcommand{\abs}[1]{\left| #1 \right|} %
\newcommand{\avg}[1]{\left< #1 \right>} %
\let\underdot=\d %
\renewcommand{\d}[2]{\frac{d #1}{d #2}} %
\newcommand{\dd}[2]{\frac{d^2 #1}{d #2^2}} %
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} 
\newcommand{\pdd}[2]{\frac{\partial^2 #1}{\partial #2^2}} 
\newcommand{\pdc}[3]{\left( \frac{\partial #1}{\partial #2}
 \right)_{#3}} %
\newcommand{\ket}[1]{\left| #1 \right>} %
\newcommand{\bra}[1]{\left< #1 \right|} %
\newcommand{\braket}[2]{\left< #1 \vphantom{#2} \right|
 \left. #2 \vphantom{#1} \right>} %
\newcommand{\matrixel}[3]{\left< #1 \vphantom{#2#3} \right|
 #2 \left| #3 \vphantom{#1#2} \right>} %
\newcommand{\grad}[1]{\gv{\nabla} #1} %
\let\divsymb=\div %
\renewcommand{\div}[1]{\gv{\nabla} \cdot \v{#1}} %
\newcommand{\curl}[1]{\gv{\nabla} \times \v{#1}} %
\let\baraccent=\= %
\renewcommand{\=}[1]{\stackrel{#1}{=}} %
\providecommand{\wave}[1]{\v{\tilde{#1}}}
\providecommand{\fr}{\frac}
\providecommand{\tbf}{\textbf}
\providecommand{\tsc}{\textsc}
\providecommand{\RR}{\mathbb{R}}
\providecommand{\R}{\mathbb{R}}
\providecommand{\NN}{\mathbb{N}}
\providecommand{\CC}{\mathbb{C}}
\providecommand{\FF}{\mathbb{F}}
\providecommand{\LL}{\mathbb{L}}
\providecommand{\ZZ}{\mathbb{Z}}
\providecommand{\QQ}{\mathbb{Q}}
\providecommand{\cA}{\mathcal{A}}
\providecommand{\cB}{\mathcal{B}}
\providecommand{\cC}{\mathcal{C}}
\providecommand{\cD}{\mathcal{D}}
\providecommand{\cE}{\mathcal{E}}
\providecommand{\cF}{\mathcal{F}}
\providecommand{\cG}{\mathcal{G}}
\providecommand{\cL}{\mathcal{L}}
\providecommand{\cM}{\mathcal{M}}
\providecommand{\cN}{\mathcal{N}}
\providecommand{\cP}{\mathcal{P}}
\providecommand{\cR}{\mathcal{R}}
\providecommand{\cS}{\mathcal{S}}
\providecommand{\cV}{\mathcal{V}}
\providecommand{\cX}{\mathcal{X}}
\providecommand{\cY}{\mathcal{Y}}
\providecommand{\sH}{\mathsf{H}}
\providecommand{\sT}{\mathsf{T}}
\providecommand{\sT}{\mathsf{T}}
\providecommand{\PP}{\mathbb{P}}
\providecommand{\EE}{\mathbb{E}}
\providecommand{\fM}{\mathfrak{M}}
\providecommand{\seq}{\subseteq}
\providecommand{\e}{\epsilon}
\providecommand{\eps}{\epsilon}
\providecommand{\de}{\delta}
\providecommand{\La}{\Lambda}
\providecommand{\N}{\mathbb{N}}
\providecommand{\la}{\lambda}
\providecommand{\al}{\alpha}
\providecommand{\Al}{\Alpha}
\providecommand{\vareps}{\varepsilon}
\providecommand{\NTIME}{\mathsf{NTIME}}
\providecommand{\DTIME}{\mathsf{DTIME}}
\providecommand{\SigmaTIME}[1]{\mathsf{\Sigma_{#1}}\mathsf{TIME}}
\providecommand{\PiTIME}[1]{\mathsf{\Pi_{#1}}\mathsf{TIME}}
\providecommand{\PH}{\mathsf{PH}}
\renewcommand{\P}{\mathsf{P}}
\providecommand{\NP}{\mathsf{NP}}
\providecommand{\NSUBEXP}{\mathsf{NSUBEXP}}
\providecommand{\NEXP}{\mathsf{NEXP}}
\providecommand{\coNP}{\mathsf{coNP}}
\providecommand{\PSPACE}{\mathsf{PSPACE}}
\providecommand{\BPP}{\mathsf{BPP}}
\providecommand{\BPNP}{\mathsf{BP}\bm{\cdot}\mathsf{NP}}
\providecommand{\DP}{\mathsf{DP}}
\providecommand{\AM}{\mathsf{AM}}
\providecommand{\VP}{\mathsf{VP}}
\providecommand{\VQP}{\mathsf{VQP}}
\providecommand{\VNP}{\mathsf{VNP}}
\providecommand{\sharpP}{\mathsf{\#P}}
\providecommand{\Ppoly}{\mathsf{P/poly}}
\providecommand{\NPpoly}{\mathsf{NP/poly}}
\providecommand{\SIZE}{\mathsf{SIZE}}
\providecommand{\ASIZE}{\mathsf{ASIZE}}
\providecommand{\PERM}{\textsc{Perm}}
\providecommand{\PIT}{\textsc{PIT}}
\providecommand{\RP}{\mathsf{RP}}
\mathchardef\mhyphen="2D %
\providecommand{\complete}{\mathsf{\mhyphen complete}}
\providecommand{\hard}{\mathsf{\mhyphen hard}}
\providecommand{\co}{\mathsf{co}}
\newcommand{\Pcc}{\mathsf{P^{cc}}}
\newcommand{\Pdt}{\mathsf{P^{dt}}}
\newcommand{\NPdt}{\mathsf{NP^{dt}}}
\newcommand{\NPcc}{\mathsf{NP^{cc}}}
\newcommand{\UPcc}{\mathsf{UP^{cc}}}
\newcommand{\UPdt}{\mathsf{UP^{dt}}}


\newcommand{\BSC}{\mathsf{BSC}}
\newcommand{\AWGN}{\mathsf{AWGN}}
\newcommand{\iid}{\stackrel{\mathrm{IID}}{\sim}}

\providecommand{\ba}{\bm{a}}
\providecommand{\bb}{\bm{b}}
\providecommand{\bc}{\bm{c}}
\providecommand{\bd}{\bm{d}}
\providecommand{\be}{\bm{e}}
\providecommand{\br}{\bm{r}}
\providecommand{\bt}{\bm{t}}
\providecommand{\bw}{\bm{w}}
\providecommand{\bx}{\bm{x}}
\providecommand{\by}{\bm{y}}
\providecommand{\bG}{\bm{G}}
\providecommand{\bQ}{\bm{Q}}

\newcommand{\dec}{{\sf Dec}}
\newcommand{\gen}{{\sf Gen}}
\newcommand{\sign}{{\sf Sign}}
\newcommand{\ver}{{\sf Ver}}
\newcommand{\pk}{{\sf pk}}


\providecommand{\sm}{\setminus}
\providecommand{\parmu}{\partial_{\mu}}
\providecommand{\parnu}{\partial_{\nu}}
\providecommand{\is}[1]{\indices{#1}}
\providecommand{\cH}{\mathcal{H}}
\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
\newcommand\chr[3]{\Gamma^{#1}_{#2 #3}}
\newcommand{\Mod}[1]{\ (\text{mod}\ #1)}
\providecommand{\del}{\nabla}
\providecommand{\gen}[1]{\langle #1 \rangle}
\newcommand{\fl}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ce}[1]{\left\lceil #1 \right\rceil}
\providecommand{\lar}{\leftarrow}
\providecommand{\rar}{\rightarrow}
\providecommand{\lrar}{\leftrightarrow}
\newcommand{\interior}[1]{%
  {\kern0pt#1}^{\mathrm{o}}%
}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\providecommand{\indy}{\independent}




\usepackage[capitalise]{cleveref}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{assumption}[theorem]{Assumption}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}



\providecommand{\cl}{\mathrm{cl}}





\providecommand{\editdist}{\mathrm{ed}}

\newcommand{\loctv}{\mathsf{locTV}}
\newcommand{\loctvk}[1]{\mathsf{locTV}^{(#1)}}
\newcommand{\muh}{{\hat \mu}}

\newcommand{\TCL}{\sT^{\mathsf{CL}}} %
\newcommand{\thetaCL}{\theta^{\mathsf{CL}}}
\providecommand{\dsT}{\dot{\sT}}
\providecommand{\tsT}{\tilde{\sT}}
\providecommand{\tsH}{\tilde{\sH}}
\providecommand{\dsH}{\dot{\sH}}
\providecommand{\hmu}{\hat{\mu}}
\providecommand{\tmu}{\tilde{\mu}}
\providecommand{\Thetah}{\hat{\Theta}}


\newcommand{\ReduceToFerromagnetic}{\texttt{LearnModel}}
\newcommand{\ReduceToLowerBounded}{\texttt{Reduce-To-Lower-Bounded}}
\newcommand{\FerromagneticSubroutine}{\texttt{LearnFerromagneticModel}}
\newcommand{\LowerboundedSubroutine}{\texttt{LowerboundedSubroutine}}
\newcommand{\ChowLiuPreprocessing}{\texttt{ChowLiuPartitioning}}
\newcommand{\LearnFerromagneticModel}{\texttt{LearnFerromagneticModel}}
\newcommand{\LearnLowerboundedModel}{\texttt{LearnLowerboundedModel}}
\newcommand{\GlobalReconstruction}{\texttt{LearnLowerboundedModel}}
\newcommand{\Desteinerize}{\texttt{Desteinerize}}

\renewcommand{\Im}{\mathrm{Im}}
\renewcommand{\Re}{\mathrm{Re}}

\newcommand{\vectorize}{\mathrm{vec}}
\newcommand{\fjunk}{f_{\mathrm{junk}}}
\newcommand{\Djunk}{\cD_{\mathrm{junk}}}
\newcommand{\elljunk}{\ell_{\Djunk}}

\newcommand{\tTheta}{\tilde{\Theta}}
\newcommand{\tilTh}{\tilde{\Theta}}
\newcommand{\tilW}{\tilde{W}}
\newcommand{\tilV}{\tilde{V}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\KL}{\mathrm{KL}}

\def\bA{{\boldsymbol A}}
\def\bB{{\boldsymbol B}}
\def\bC{{\boldsymbol C}}
\def\bD{{\boldsymbol D}}
\def\bE{{\boldsymbol E}}
\def\bF{{\boldsymbol F}}
\def\bG{{\boldsymbol G}}

\def\bH{{\boldsymbol H}}
\def\bI{{\boldsymbol I}}
\def\bJ{{\boldsymbol J}}
\def\bK{{\boldsymbol K}}
\def\bL{{\boldsymbol L}}
\def\bM{{\boldsymbol M}}
\def\bN{{\boldsymbol N}}
\def\bO{{\boldsymbol O}}
\def\bP{{\boldsymbol P}}
\def\bQ{{\boldsymbol Q}}
\def\bR{{\boldsymbol R}}
\def\bS{{\boldsymbol S}}
\def\bT{{\boldsymbol T}}
\def\bU{{\boldsymbol U}}
\def\bV{{\boldsymbol V}}
\def\bW{{\boldsymbol W}}
\def\bX{{\boldsymbol X}}
\def\bY{{\boldsymbol Y}}
\def\bZ{{\boldsymbol Z}}

\def\ba{{\boldsymbol a}}
\def\bb{{\boldsymbol b}}
\def\be{{\boldsymbol e}}
\def\boldf{{\boldsymbol f}}
\def\bg{{\boldsymbol g}}
\def\bh{{\boldsymbol h}}
\def\bi{{\boldsymbol i}}
\def\bj{{\boldsymbol j}}
\def\bk{{\boldsymbol k}}
\def\bq{{\boldsymbol q}}
\let\bsold\bs
\def\bs{{\boldsymbol s}}
\def\bt{{\boldsymbol t}}
\def\bu{{\boldsymbol u}}
\def\bv{{\boldsymbol v}}
\def\bw{{\boldsymbol w}}
\def\bx{{\boldsymbol x}}
\def\by{{\boldsymbol y}}
\def\bz{{\boldsymbol z}}

\def\bbeta{{\boldsymbol \beta}}
\def\balpha{{\boldsymbol \alpha}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol \eps}}
\def\blambda{{\boldsymbol \lambda}}
\def\bpsi{{\boldsymbol \psi}}
\def\bphi{{\boldsymbol \phi}}
\def\btheta{{\boldsymbol \theta}}
\def\tbtheta{\tilde{\btheta}}
\def\bvphi{{\boldsymbol \vphi}}
\def\bxi{{\boldsymbol \xi}}

\def\bDelta{{\boldsymbol \Delta}}
\def\bLambda{{\boldsymbol \Lambda}}
\def\bPsi{{\boldsymbol \Psi}}
\def\bPhi{{\boldsymbol \Phi}}
\def\bSigma{{\boldsymbol \Sigma}}
\def\bTheta{{\boldsymbol \Theta}}
\def\bzeta{{\boldsymbol \zeta}}

\def\bzero{{\boldsymbol 0}}
\def\bfzero{{\boldsymbol 0}}
\def\bfone{{\boldsymbol 1}}
\def\bone{{\boldsymbol 1}}


\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}

\newcommand{\fNN}{f_{\mathsf{NN}}}
\newcommand{\tfNN}{\tilde{f}_{\mathsf{NN}}}
\newcommand{\gNN}{g_{\mathsf{NN}}}

\newcommand{\barcF}{\bar{\cF}}

\newcommand{\fparity}{f_{\mathrm{parity}}}
\newcommand{\fmodeight}{f_{\mathrm{mod8}}}
\newcommand{\cDmodeight}{\cD_{\mathrm{mod8}}}

\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}

\newenvironment{algbox}[0]{
\noindent 
\begin{fminipage}{4.7in}
}{
\end{fminipage}
}


\newcommand{\ud}{\mathrm{d}}
\newcommand{\sig}{\sigma}
